$C-(k, \ell)$-Sum-Free Sets

The Minkowski sum of two subsets $A$ and $B$ of a finite abelian group $G$ is defined as all pairwise sums of elements of $A$ and $B$: $A + B = \{ a + b : a \in A, b \in B \}$. The largest size of a $(k, \ell)$-sum-free set in $G$ has been of interest for many years and in the case $G = \mathbb{Z}/n\mathbb{Z}$ has recently been computed by Bajnok and Matzke. Motivated by sum-free sets of the torus, Kravitz introduces the noisy Minkowski sum of two sets, which can be thought of as discrete evaluations of these continuous sumsets. That is, given a noise set $C$, the noisy Minkowski sum is defined as $A +_C B = A + B + C$. We give bounds on the maximum size of a $(k, \ell)$-sum-free subset of $\mathbb{Z}/n\mathbb{Z}$ under this new sum, for $C$ equal to an arithmetic progression with common difference relatively prime to $n$ and for any two element set $C$.

==> 01-c-equality.tex <==
\section{Equality}



\begin{lemma}
    For $C = \{ 0, 1, \dots, c-1 \}$ and any subset $A \subseteq \mathbb{Z}/n\mathbb{Z}$, if $A$ contains two elements $x$ and $y$ such that $y - x < c - \lceil \frac{c-2}{k} \rceil$, then $k *_C (A \cup \{ z \}) = k *_C A$ for any $z \in \{ x+1, \dots, y-1 \}$.
\end{lemma}

\begin{proof}
    Suppose that there are elements $x, y \in A$ such that $2 \le y - x < c - \lceil \frac{c-2}{k} \rceil$. Then, for any $z \in \{ x+1, \dots, y-1 \}$, the set $k *_C (A \cup \{ z \})$ can be written as
    \[
        \{ a_1 + \dots + a_k + b \ |\ a_i \in A \cup \{ z \}, b \in \{ 0, 1, \dots, (k-1)(c-1) \} \}.
    \]
    Since any $a_1 + \dots + a_k + b$ with all $a_i \in A$ is already in $k *_C A$, it suffices to show that any such sum with at least one of the $a_i$ equal to $z$ is also in $k *_C A$.
    
    To do this, consider a sum $a_1 + \dots + a_k + b$, where $j$ of the $a_i$'s are equal to $z$. Then, consider replacing every of the $j$ instances of $z$ with $x$, and with $y$. In the first case, the value of $a_1 + \dots + a_k + b$ decreases by at most $k(z-x)$, and in the second, the value increases by at most $k(y-z)$. Since $k(z-x) + k(y-z) = k(y-x) \le k(c - 1 - \lceil \frac{c-2}{k} \rceil) \le (k-1)(c-1) - 1$, we have that either $b$ is at least $k(y-z) + 1$, in which case $b' = b - j(y-z) \in \{ 0, 1, \dots, (k-1)(c-1) \}$, or $b$ is at most $(k-1)(c-1) - k(z-x)$, in which case $b' = b + j(z-x) \in \{ 0, 1, \dots, (k-1)(c-1) \}$. In the first case, $a_1 + \dots + a_k + b$ is equal to $a'_1 + \dots + a'_k + b'$, where $a'_i = a_i$ if $a_i \not= z$, otherwise $a'_i = y$; in the second, $a_1 + \dots + a_k + b$ is equal to $a'_1 + \dots + a'_k + b'$, where $a'_i = a_i$ if $a_i \not= z$ and $a'_i = x$ otherwise. Since we can always rewrite $a_1 + \dots + a_k + b$ with elements of $A$, we have that $k *_C (A \cup \{ z \}) = k *_C A$.
\end{proof}




Let $A$ be a maximal $C$-$(k, \ell)$-sum-free set in $\mathbb{Z}/n\mathbb{Z}$. Noting that single elements are also intervals, we can write any set as a union of disconnected intervals. The fact that $A$ is $C$-$(k, \ell)$-sum-free allows us to say a bit more about the distance between these intervals.




==> 0p-bounds.tex <==
\section{Maximal $\{ 0, p \}$-$(k, \ell)$-Sum-Free Sets}

We now restrict our attention to $C$ of size $2$. First, by shifting, we can write $C$ as $\{ 0, c \}$. When $c$ is relatively prime to $n$, we can multiply $C$ by $c^{-1}$ so that $C = \{ 0, 1 \}$, which we have understood in the previous section. Therefore, we now consider sets $C = \{ 0, c \}$ for which $\gcd(c, n) \not= 1$. In particular, we look at $C = \{ 0, p \}$ where $p$ is a prime and $p | n$. 

\begin{theorem}\label{thm:0p-main}
    When $p | k - \ell$, 
    \[
        \left\lfloor \frac{n + 2(p-1) - r}{k + \ell} \right\rfloor - (p - 1)
        \le \mu_{k, \ell}^{\{ 0, p \}}(\mathbb{Z}/n\mathbb{Z}) 
        \le \left\lfloor \frac{n}{k + \ell} \right\rfloor,
    \]
    and when $p \not| k - \ell$, 
    \[
        \max \left\{ \left\lceil \frac{p - 1}{k + \ell} \right\rceil \cdot \frac{n}{p},\ \left\lfloor \frac{n + 2(p-1) - r}{k + \ell} \right\rfloor - (p - 1) \right\}
        \le \mu_{k, \ell}^{\{ 0, p \}}(\mathbb{Z}/n\mathbb{Z}) 
        \le \max \left\{ \left\lceil \frac{p - 1}{k + \ell} \right\rceil \cdot \frac{n}{p},\ \left\lfloor \frac{n}{k + \ell} \right\rfloor \right\},
    \]
    where $\delta = \gcd(n, k - \ell)$, $f = \lfloor \frac{n + 2(p-1)}{k + \ell} \rfloor - (p-1)$, and $r$ is the residue of $-kf - (k-1)(p-1)$ modulo $\delta$. 
\end{theorem}

Note for instance that if $p \not| k - \ell$ and $\lceil \frac{p - 1}{k + \ell} \rceil \cdot \frac{n}{p} \ge \lfloor \frac{n}{k + \ell} \rfloor$, then we in fact have equality: 
\[
    \mu_{k, \ell}^{\{ 0, p \}}(\mathbb{Z}/n\mathbb{Z})
    = \left\lceil \frac{p - 1}{k + \ell} \right\rceil \cdot \frac{n}{p}.
\]

In order to prove this theorem, we will prove the lower and upper bounds separately. The lower bound will follow from the following lemma:

\begin{lemma}
    For any $k > \ell$, 
    \[
        \mu_{k, \ell}^{\{ 0, p \}}(\mathbb{Z}/n\mathbb{Z})
        \ge \max \left\{ 
            \mu_{k, \ell}(\mathbb{Z}/p\mathbb{Z}) \cdot \frac{n}{p},\ 
            \mu_{k, \ell}^{\{ 0, 1, \dots, p \}}(\mathbb{Z}/n\mathbb{Z}) 
        \right\}.
    \]
\end{lemma}

\begin{proof}
    First, suppose that we have a $(k, \ell)$-sum-free set $B$ in $\mathbb{Z}/p\mathbb{Z}$, and define $\psi_{n, p}$ to be the canonical projection from $\mathbb{Z}/n\mathbb{Z}$ to $\mathbb{Z}/p\mathbb{Z}$. Then, $A = \psi_{n, p}^{-1}(B)$ must also be $(k, \ell)$-sum-free and in fact $\{ 0, p \}$-$(k, \ell)$-sum-free. Since $A$ has size $\mu_{k, \ell}(\mathbb{Z}/p\mathbb{Z}) \cdot \frac{n}{p}$, the first lower bound is established.
    
    Next, we have that $\{ 0, p \} \subseteq \{ 0, 1, \dots, p \}$, so any $\{ 0, 1, \dots, p \}$-$(k, \ell)$-sum-free set in $\mathbb{Z}/n\mathbb{Z}$ must also be a $\{ 0, p \}$-$(k, \ell)$-sum-free set in $\mathbb{Z}/n\mathbb{Z}$. This gives the second of the two lower bounds.
    
    Since $\mu_{k, \ell}^{\{ 0, p \}}(\mathbb{Z}/n\mathbb{Z})$ is lower bounded by both $\mu_{k, \ell}(\mathbb{Z}/p\mathbb{Z})\cdot \frac{n}{p}$ and $\mu_{k, \ell}^{\{ 0, 1, \dots, p \}}(\mathbb{Z}/n\mathbb{Z})$, we have that it is at least the maximum of the two.
\end{proof}

Now, from Bier and Chin we know that 
\[
    \mu_{k, \ell}(\mathbb{Z}/p\mathbb{Z}) = \begin{cases}
        \left\lceil \frac{p - 1}{k + \ell} \right\rceil & p \not| k - \ell \\
        0 & p | k - \ell
    \end{cases}.
\]
Using this result and the lower bound in Theorem~\ref{thm:01c-main}, we get the lower bound in Theorem~\ref{thm:0p-main}. 

In order to handle the upper bound, we need a few lemmas.

\begin{lemma} \label{lemma:substab}
    For sets $A$ and $B$, $\stab(A) \subseteq \stab(A + B)$ as a subgroup inclusion.
\end{lemma}

\begin{proof}
    We have that 
    \[
        \stab(A) + (A + B)
        = (\stab(A) + A) + B 
        = A + B.
    \]
\end{proof}

We can write $A +_C B = A + B + C$, so this lemma also gives that $\stab(A) \subseteq \stab(A +_C B)$. 

\begin{lemma} \label{lemma:0p-bound-stab-not-p}
    For a $\{ 0, p \}$-$(k, \ell)$-sum-free set $A$, let $K = \stab(k *_{\{ 0, p \}} A)$ and suppose that $K \not= \langle p \rangle$. Then
    \[
        |A| \le \left\lfloor \frac{n}{k + \ell} \right\rfloor. 
    \]
\end{lemma}

\begin{proof}
    Our proof of this lemma follows from the following claim.
    
    Claim:
        For all $1 \le j \le k$, $|j *_{\{ 0, p \}} A| \ge j |A|$. 
        
    We prove this claim via induction. For $j = 1$, $|j *_{\{ 0, p \}} A| = |A|$, so the base case is true. Now for $2 \le j \le k$, suppose the claim is true for $j - 1$. Let $J = \stab(j *_{\{ 0, \}} A)$. By Kneser, we have that 
    \[
        |j *_{\{ 0, p \}} A|
        \ge |A + ((j - 1) *_{\{ 0, p \}} A)| + |\{ 0, p \} + J| - |J|.
    \]
    By Lemma~\ref{lemma:substab}, $J$ is a subgroup of $K$, so $J \not= \langle p \rangle$. Also, $J \not= \langle 1 \rangle$ otherwise $j *_{\{ 0, p \}} A = \mathbb{Z}/n\mathbb{Z} \implies k *_{\{ 0, p \}} A = \mathbb{Z}/n\mathbb{Z}$, contradicting the fact that $A$ is a $\{ 0, p \}$-$(k, \ell)$-sum-free. Then, we have that $|\{ 0, p \} + J| = 2|J|$, so we can rewrite the above equation as 
    \begin{align*}
        |j *_{\{ 0, p \}} A|
        &\ge |A + ((j - 1) *_{\{ 0, p \}} A)| + |J| \\
        &\ge |A| + |(j - 1) *_{\{ 0, p \}} A| + |J| - |H| \\
        &\ge |A| + |(j - 1) *_{\{ 0, p \}} A| \\
        &\ge |A| + (j-1) |A| \\
        &= j |A|,
    \end{align*}
    where $H = \stab(A + ((j - 1) *_{\{ 0, p \}} A)) \subseteq J$ by Lemma~\ref{lemma:substab}, so $|H| \le |J|$. This completes the proof of the claim.
    
    To finish our proof, we have that $|k *_{\{ 0, p \}} A| \ge k |A|$ and $|\ell *_{\{ 0, p \}} A| \ge \ell |A|$. Since $k *_{\{ 0, p \}} A \cap \ell *_{\{ 0, p \}} A = \emptyset$, we have that $n \ge (k + \ell)|A| \implies |A| \le \lfloor \frac{n}{k + \ell} \rfloor$. 
\end{proof}

Now, we are ready to prove the upper bound.

\begin{lemma}
    For any $k > \ell$, 
    \[
        \mu_{k, \ell}^{\{ 0, p \}}(\mathbb{Z}/n\mathbb{Z}) 
        \le \max \left\{ 
            \mu_{k, \ell}(\mathbb{Z}/p\mathbb{Z}) \cdot \frac{n}{p},\ 
            \left\lfloor \frac{n}{k + \ell} \right\rfloor
        \right\}.
    \]
\end{lemma}

\begin{proof}
    Suppose that $A$ is a $\{ 0, p \}$-$(k, \ell)$-sum-free set in $\mathbb{Z}/n\mathbb{Z}$. Once again define the map $\psi_{n, p}$ to be the canonical projection onto $\mathbb{Z}/p\mathbb{Z}$. We consider cases based on $|\psi_{n, p}(A)|$, the number of distinct residues elements of $A$ leave modulo $p$.
    
    First, suppose $|\psi_{n, p}(A)| > \mu_{k, \ell}(\mathbb{Z}/p\mathbb{Z})$. Then, if $K = \stab(k *_{\{ 0, p \}} A) = \langle p \rangle$, we have that $k *_{\{ 0, p \}} A$ is a union of cosets of $\langle p \rangle$ but is not equal to $\mathbb{Z}/n\mathbb{Z}$. Since $\psi_{n, p}(k *_{\{0, p \}} A) = k \psi_{n, p}(A)$ and $|\psi_{n, p}(A)| > \mu_{k, \ell}(\mathbb{Z}/p\mathbb{Z})$, then $k \psi_{n, p}(A) \cap \ell \psi_{n, p}(A) \not= \emptyset$. However, since $k *_{\{ 0, p \}} = \psi_{n, p}^{-1}(\psi_{n, p}(A))$ is a union of cosets, it must have nontrivial intersection with $\ell *_{\{ 0, p \}} A$, contradiction on $A$ being $\{ 0, p \}$-$(k, \ell)$-sum-free. Then, assume $K \not= \langle p \rangle$, in which case Lemma~\ref{lemma:0p-bound-stab-not-p} gives that $|A| \le \lfloor \frac{n}{k + \ell} \rfloor$.
    
    Now, suppose $|\psi_{n, p}(A)| \le \mu_{k, \ell}(\mathbb{Z}/p\mathbb{Z})$. Since $|\psi_{n, p}^{-1}(\{ a \})| = \frac{n}{p}$ for any element $a \in \mathbb{Z}/p\mathbb{Z}$, we have that $|A|$ is upper bounded by $\mu_{k, \ell}(\mathbb{Z}/p\mathbb{Z}) \cdot \frac{n}{p}$. 
    
    Combining the upper bounds in the two cases gives that $\mu_{k, \ell}^{\{ 0, p \}}(\mathbb{Z}/n\mathbb{Z})$ is upper bounded by the larger of the two.
\end{proof}

The upper bounds in Theorem~\ref{thm:0p-main} can be found by using the fact that $\mu_{k, \ell}(\mathbb{Z}/p\mathbb{Z}) = \lceil \frac{p - 1}{k + \ell} \rceil$ when $p \not| k - \ell$ and $0$ when $p | k - \ell$.



==> 2elt-bounds.tex <==
\section{$C$ of size $2$}

Note that if $C$ is of size $1$, we can reduce the question to asking about $C = \{ 0 \}$, in which case $+_C$ is the same as the Minkowski sum, which has been thoroughly investigated. Thus, we first consider $C$ of size $2$.

If $C$ is of size $2$, we can without loss of generality assume $C = \{ 0, c \}$ by Proposition~\ref{prop:shift}, and we can divide out by $\frac{c}{\gcd(n, c)}$ by Proposition~\ref{prop:mult}, so we may assume that $C = \{ 0, c \}$ where $c | n$. In the case $c = 1$, which corresponds to original $C$ of two elements whose difference is relatively prime to $n$, we have the following result, which partially answers Kravitz's question.

\begin{theorem}
    With $\delta = \gcd(n, k - \ell)$ and $r$ equal to the remainder of $-\lfloor \frac{n}{k + \ell} \rfloor \cdot k$ modulo $\delta$, we have the following bounds:
    \[
        \left\lfloor \frac{n - r}{k + \ell} \right\rfloor 
        \le \mu_{k, \ell}^{\{ 0, 1 \}} (\mathbb{Z}/n\mathbb{Z})
        \le \left\lfloor \frac{n}{k + \ell} \right\rfloor.
    \]
\end{theorem}

Note that this handles the case $n | k - \ell$: when $n | k - \ell$, then any nonempty $A$ has $kA \cap \ell A \not= \emptyset$ since $ka = \ell a$ for any $a \in \mathbb{Z}/n\mathbb{Z}$. Then, $\mu_{k, \ell}^{\{ 0, 1 \}}(\mathbb{Z}/n\mathbb{Z}) = 0$. But if $n | k - \ell$, then $n \le k - \ell < k + \ell$, so the upper bound in the theorem is $\lfloor \frac{n}{k + \ell} \rfloor = 0$. 

To prove the theorem, we will prove the upper and lower bounds separately. The upper bound depends on a bound on $(k, \ell)$-sum-free sets in the torus. To talk about sum-free sets on the torus, let $\mu^*$ denote the normalized Haar measure on the torus $\mathbb{T}$ and let $\mu_{k, \ell}^*(\mathbb{T}) = \max \{ \mu^*(A)\ |\ A \subseteq \mathbb{T}, kA \cap \ell A = \emptyset \}$. Then, Kravitz proved the following:

\begin{theorem} \emph{(Kravitz, 2019)}
    $\mu_{k, \ell}^*(\mathbb{T}) = \frac{1}{k + \ell}$.
\end{theorem}

As a result, we derive the following upper bound on $\mu_{k, \ell}^{\{ 0, 1 \}}(\mathbb{Z}/n\mathbb{Z})$.

\begin{theorem}
    $\mu_{k, \ell}^{\{ 0, 1 \}} \le \left\lfloor \frac{n}{k + \ell} \right\rfloor$. 
\end{theorem}

\begin{proof}
    For any $A \subseteq \mathbb{Z}/n\mathbb{Z}$, consider the map $\phi : \mathcal{P}(\mathbb{Z}/n\mathbb{Z}) \rightarrow \mathcal{P}(\mathbb{T})$ defined by $\phi(A) = \bigcup_{i \in A} \left( \frac{i}{n}, \frac{i + 1}{n} \right)$. We have that since $\left( \frac{i}{n}, \frac{i + 1}{n} \right) + \left( \frac{j}{n}, \frac{j + 1}{n} \right) = \left( \frac{i + j}{n}, \frac{i + j + 2}{n} \right)$, then $\phi( A +_{\{ 0, 1 \}} B ) = \phi(A) + \phi(B)$. Therefore, $A$ is $\{ 0, 1 \}$-$(k, \ell)$-sum-free iff $\phi(A)$ is sum-free. Then,
    \[
        \mu_{k, \ell}^{\{ 0, 1 \}}(\mathbb{Z}/n\mathbb{Z}) 
        \le n \cdot \mu^*_{k, \ell}(\mathbb{T}) 
        = \frac{n}{k + \ell}.
    \]
    Since $\mu_{k, \ell}^{\{ 0, 1 \}}(\mathbb{Z}/n\mathbb{Z})$ is an integer, we in fact have that 
    \[
        \mu_{k, \ell}^{\{ 0, 1 \}}(\mathbb{Z}/n\mathbb{Z})
        \le \left\lfloor \frac{n}{k + \ell} \right\rfloor.
    \]
\end{proof}

\begin{theorem}
    $\mu_{k, \ell}^{\{ 0, 1 \}} \ge \lfloor \frac{n - r}{k + \ell} \rfloor$, where $\delta = \gcd(n, k - \ell)$ and $r$ is the residue of $-\lfloor \frac{n}{k + \ell} \rfloor \cdot k$ modulo $\delta$. 
\end{theorem}

\begin{proof}
    To see this lower bound, we provide a construction of a set of $\lfloor \frac{n - r}{k + \ell} \rfloor$ elements of $\mathbb{Z}/n\mathbb{Z}$ that is $\{ 0, 1 \}$-$(k, \ell)$-sum-free. In particular, we will restrict to intervals.
    
    Consider an interval $A = [a, \cdots, a + m - 1]$ of $m$ elements of $\mathbb{Z}/n\mathbb{Z}$. Then, $k *_{\{ 0, 1 \}} A = [ka, \dots, ka + km - 1]$ and $\ell *_{\{ 0, 1 \}} A = [\ell a, \dots, \ell a + km - 1]$. Then, $k *_{\{ 0, 1 \}} A \cap \ell *_{\{ 0, 1 \}} A = \emptyset$ iff $k *_{\{ 0, 1 \}} A - \ell *_{\{ 0, 1 \}} = [(k-\ell)a - m\ell + 1, (k-\ell)a + mk - 1]$ does not contain $0$, that is, there exists some integer $b$ for which 
    \begin{align*}
        (k - \ell)a - m\ell + 1 &\ge bn + 1 \\
        (k - \ell)a + mk - 1 &\le (b + 1)n - 1.
    \end{align*} 
    This can be rewritten as 
    \[
        m\ell 
        \le (k - \ell)a - bn 
        \le n - mk.
    \]
    Let $\delta = \gcd(n, k - \ell)$, so we may write
    \[
        \frac{m\ell}{\delta}
        \le \frac{k - \ell}{\delta}\cdot a - \frac{n}{\delta} \cdot b 
        \le \frac{n - mk}{\delta}.
    \]
    Since $\gcd \left( \frac{k - \ell}{\delta}, \frac{n}{\delta} \right) = 1$, any integer can be written as $\frac{k - \ell}{\delta} \cdot a - \frac{n}{\delta} \cdot b$ for some $a, b \in \mathbb{Z}$. Thus, there exists a $\{ 0, 1 \}$-$(k, \ell)$-sum-free interval of length $m$ iff there exists some integer $Z$ for which 
    \[
        \frac{m\ell}{\delta} \le Z \le \frac{n - mk}{\delta},
    \]
    that is,
    \[
        \frac{m\ell}{\delta} 
        \le \left\lfloor \frac{n - mk}{\delta} \right\rfloor.
    \]
    Let $m^*$ denote the largest integer solution to this inequality. We have that $\lfloor \frac{n - mk}{\delta} \rfloor \ge \frac{n - mk - \delta + 1}{\delta}$, which is at least $\frac{m\ell}{\delta}$ when $m \le \frac{n - \delta + 1}{k + \ell}$, or $m^* = \lfloor \frac{n - \delta + 1}{k + \ell} \rfloor$. Since $\delta = \gcd(n, k - \ell) \le k - \ell < k + \ell$, we have that $m^*$ equals either $\lfloor \frac{n}{k + \ell} \rfloor$ or $\lfloor \frac{n}{k + \ell} \rfloor - 1$. 
    
    Let $f = \lfloor \frac{n}{k + \ell} \rfloor$. Letting $r$ denote the residue of $k \lfloor \frac{n}{k + \ell} \rfloor$ modulo $\delta$, we have that $\lfloor \frac{n - fk}{\delta} \rfloor = \frac{n - fk - r}{\delta}$, so $m^* = f$ iff
    \[
        f\ell \le n - fk - r 
        \Longleftrightarrow 
        f \le \frac{n - r}{k + \ell}.
    \]
    This is the same as letting $m^* = \lfloor \frac{n - r}{k + \ell} \rfloor$. 
\end{proof}

\begin{corollary}
    If $\gcd(n, k - \ell) = 1$, then $\mu_{k, \ell}^{\{ 0, 1 \}} = \lfloor \frac{n}{k + \ell} \rfloor$. In particular, if $n = p$ is prime and $p \not| k - \ell$, then $\mu_{k, \ell}^{\{ 0, 1 \}} = \lfloor \frac{p}{k + \ell} \rfloor$. 
\end{corollary}

Next, suppose that $c > 1$. We have the following bounds:

\begin{theorem}
    In the following, let $\delta = \gcd(d, k - \ell)$ and $r$ be the remainder of $\ell \cdot \left\lceil \frac{d - \delta}{k + \ell} \right\rceil \Mod{\delta}$. Then,
    \[
        \max_{d | c} \left\{ \left\lceil \frac{d - (\delta - r)}{k + \ell} \right\rceil \cdot \frac{n}{d} \right\} 
        \le \mu_{k, \ell}^C (\mathbb{Z})
        \le \max_{d | n} \left\{ \left\lfloor \frac{d + \frac{2|C| d}{n} - 4}{k + \ell} - \frac{|C| d}{n} + 2 \right\rfloor \cdot \frac{n}{d} \right\}
    \]
\end{theorem}

The upper bound here is a slight improvement upon the obvious upper bound given by the fact that any $C$-$(k, \ell)$-sum-free subset is also $(k, \ell)$-sum-free. 

\begin{proof}
    To see the lower bound, note that if we have a $(k, \ell)$-sum-free subset $B$ of $\mathbb{Z}_c$, then this naturally lifts to a $C$-$(k, \ell)$-sum-free set (by taking all elements of $\mathbb{Z}/n\mathbb{Z}$ that are congruent to an element of $B$ modulo $c$). Combining with Bajnok and Matzke's result, we get the lower bound.
    
    As for the upper bound, we first show a few properties about the stabilizer of $k *_C A$, if $A$ is a $C$-$(k, \ell)$-sum-free set of maximal size. Let $K$ be the stabilizer of $k *_C A$. Then, $k *_C (A + K) = k *_C A + kK = k *_C A$, so $A + K$ is $C$-$(k, \ell)$-sum-free as well. Then, since $A$ is of maximal size and $A = A + \{ 0 \} \subseteq A + K$, we have in fact that $A = A + K$. Finally, we have that $a + K \subseteq A + K = A$, so $A$ is a union of cosets of $K$. In particular, $\frac{|A|}{|K|} \in \mathbb{Z}$.
    
    We have by Kneser that $|k *_C A| \ge k|A| + (k-1)|C| - (2k-2)|\stab(k *_C A)|$ and $|\ell *_C A| \ge \ell |A| + (\ell - 1)|C| - (2\ell - 2)|\stab(\ell *_C A)|$. Suppose without loss of generality that $|\stab(k *_C A)| \ge |\stab(\ell *_C A)|$, and let $K = \stab(k *_C A)$. Then, 
    \begin{align*}
        n 
        &\ge |k *_C A| + |\ell *_C A| \\
        &= (k + \ell)|A| + (k + \ell - 2)|C| - (2k + 2\ell - 4)|K| \\
        \Longleftrightarrow 
        \frac{|A|}{|K|}
        &\le \frac{n - (k + \ell - 2)|C| + (2k + 2\ell - 4)|K|}{(k + \ell)|K|}.
    \end{align*}
    Letting $|K| = \frac{n}{d}$, we have that
    \[
        \frac{|A|}{|K|}
        \le \frac{d + \frac{2d|C|}{n} - 4}{k + \ell} - \frac{d|C|}{n} + 2.
    \]
    Since $\frac{|A|}{|K|}$ is an integer, we have that 
    \[
        |A| 
        \le \left\lfloor \frac{d + \frac{2d|C|}{n} - 4}{k + \ell} - \frac{d|C|}{n} + 2 \right\rfloor \cdot \frac{n}{d},
    \]
    as claimed.
\end{proof}


==> 3elt-bounds.tex <==
\section{$C$ of size $3$}

We move on to consider sets of size $3$. We first classify which sets can be related by a sequence of shifts and multiplications.

\begin{lemma}
    $C$ and $D$ are related by a sequence of shifts and multiplications iff $D = g(C + \{ h \})$ for some elements $h \in \mathbb{Z}/n\mathbb{Z}$ and $g \in \mathbb{Z}/n\mathbb{Z}^\times$. 
\end{lemma}

\begin{proof}
    It suffices to show that a multiplication followed by a shift can be rewritten as a shift followed by a multiplication, as then we can group all the shifts first and multiplications second. Then, since a composition of shifts is a shift and a composition of multiplications is a multiplication, the result follows. 
    
    To see this, suppose we $D = gC + h$ for some $g \in \mathbb{Z}/n\mathbb{Z}^\times$ and $h \in \mathbb{Z}/n\mathbb{Z}$. We can rewrite this as $D = g(C + \frac{h}{g})$, which is a shift followed by a multiplication. Since $g$ is a unit, we have that $\frac{h}{g}$ is defined, so $D$ is also the result of a shift by $\frac{h}{g}$ followed by a multiplication by $g$.
\end{proof}

Now, assume $n = p$ is a prime. Via shift and multiplication, we can write any set $C$ of size $3$ as $\{ 0, 1, c \}$. 

\begin{lemma}
    Sets $C = \{ 0, 1, c \}$ and $D = \{ 0, 1, d \}$ are related by a sequence of shifts and multiplications iff 
    \[
        d \in \left\{ c, \frac{1}{c}, -(c-1), -\frac{1}{c-1}, \frac{c-1}{c}, \frac{c}{c-1} \right\}.
    \]
\end{lemma}

